Multimodal Generalized Category Discovery

Generalized Category Discovery (GCD) aims to classify inputs into both known and novel categories, a task crucial for open-world scientific discoveries. However, current GCD methods are limited to unimodal data, overlooking the inherently multimodal nature of most real-world data. In this work, we extend GCD to a multimodal setting, where inputs from different modalities provide richer and complementary information. Through theoretical analysis and empirical validation, we identify that the key challenge in multimodal GCD lies in effectively aligning heterogeneous information across modalities. To address this, we propose MM-GCD, a novel framework that aligns both the feature and output spaces of different modalities using contrastive learning and distillation techniques. MM-GCD achieves new state-of-the-art performance on the UPMC-Food101 and N24News datasets, surpassing previous methods by 11.5\% and 4.7\%, respectively.

==> tables/main_table.tex <==
\begin{table}[!tb]

\vspace{-1em}
\begin{center}
\setlength{\tabcolsep}{4pt} % 调整列间距
\renewcommand{\arraystretch}{0.9} % 调整行间距
\resizebox{0.47\textwidth}{!}{%
\begin{tabular}{lcccccccc}
\toprule
& & &  \multicolumn{3}{c}{Food101} & \multicolumn{3}{c}{N24News}\\
\cmidrule(rl){4-6} \cmidrule(rl){7-9}
Methods & Sup  & Modal   & All  & Old  & New  & All  & Old  & New  \\
\midrule
\emph{MMBT} \shortcite{kiela2020supervisedmultimodalbitransformersclassifying} & \ding{51} & Fusion & \emph{92.1} & - & - & - & - & - \\ 
\emph{CMA-CLIP} \shortcite{liu2021cma} & \ding{51} & Fusion & \emph{93.1} & - & - & - & - & - \\ 
\emph{UniS-MMC} \shortcite{zou2023unismmc}  & \ding{51} & Fusion & \emph{94.7} & - & - & 84.7 & - & - \\ 
\midrule
\multirow{3}{*}{GCD~\shortcite{Vaze_2022_CVPR}} & \multirow{3}{*}{\ding{55}} & Visual & 40.0 & 68.7 & 25.3 & 27.8 & 30.1 & 27.0  \\ 
& & Text & 68.7 & 79.5 & 63.2 & 33.1 & 43.3 & 26.9 \\
& & Fusion & 61.7 & 75.5 & 54.8 & 32.8 & 44.2 & 26.0 \\
\midrule
\multirow{3}{*}{SimGCD~\shortcite{Wen_2023_ICCV}}  & \multirow{3}{*}{\ding{55}} & Visual & 65.5 & 75.0 & 60.8 & 44.7 & 54.0 & 39.2  \\ 
& & Text & 80.8 & 84.3 & 79.1 & 62.0 & \textbf{75.2} & 54.0 \\
& & Fusion & 73.1 & 85.7 & 66.8 & 63.8 & 75.1 & 57.1 \\
\midrule

{SPTNet~\shortcite{wang2024sptnet}}  & {\ding{55}} & Visual & 64.5& 71.4 & 61.0 & 44.1 & 53.5 & 38.5  \\ 
\midrule

{DPN ~\shortcite{an2023generalizedcategorydiscoverydecoupled}}  & {\ding{55}} & Text & 75.4 & 81.3 & 69.7 & 59.5 & 69.7 & 50.7  \\ 
\midrule
\multirow{3}{*}{Ours}                    & \multirow{3}{*}{\ding{55}} & Visual & 85.5 & 92.5 & 82.0 & 64.8 & 69.2 & 62.6  \\ 
& & Text & 85.3 & 92.3 & 81.9  & 65.1 & 68.9 & 62.8 \\
& & Fusion & \textbf{92.3} & \textbf{92.9} & \textbf{92.0} & \textbf{68.5} & 74.8 & \textbf{64.5} \\
\bottomrule
\end{tabular}%
}
\vspace{-1em}
\caption{Results on the UPMC-Food101 Dataset~\cite{wang2015recipe} and N24News Dataset \cite{wang-etal-2022-n24news}.}
\label{tab:main_result}
\vspace{-1em}
\end{center}
\end{table}
